DeepAlloc: CNN-Based Approach to Efficient Spectrum Allocation in Shared Spectrum Systems

Shared spectrum systems facilitate spectrum allocation to unlicensed users without harming the licensed users; they offer great promise in optimizing spectrum utility, but their management (in particular, efficient spectrum allocation to unlicensed users) is challenging. A significant shortcoming of current allocation methods is that they are either done very conservatively to ensure correctness, or are based on imperfect propagation models and/or spectrum sensing with poor spatial granularity. This leads to poor spectrum utilization, the fundamental objective of shared spectrum systems. To allocate spectrum near-optimally to secondary users in general scenarios, we fundamentally need to have knowledge of the signal path-loss function. In practice, however, even the best known path-loss models have unsatisfactory accuracy, and conducting extensive surveys to gather path-loss values is infeasible. To circumvent this challenge, we propose to learn the spectrum allocation function directly using supervised learning techniques. We particularly address the scenarios when the primary users' information may not be available; for such settings, we make use of a crowdsourced sensing architecture and use the spectrum sensor readings as features. We develop an efficient CNN-based approach (called DeepAlloc) and address various challenges that arise in its application to the learning the spectrum allocation function. Via extensive large-scale simulation and a small testbed, we demonstrate the effectiveness of our developed techniques; in particular, we observe that our approach improves the accuracy of standard learning techniques and prior work by up to 60%.

==> sections/cnn_model_fig.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[t]{1\textwidth}
   \includegraphics[width=\textwidth, center]{figures/cnn_model.png}
   \vspace*{-0.6cm}
      \caption{\blue{\name} Model for Spectrum Allocation.}
   \label{fig:cnn_model}
  \vspace*{-0.2cm}
\end{minipage}
\hspace{0.1in}
  \vspace{-0.1in}
\end{figure*}

==> sections/eaten.tex <==
\X \in \mathbb{R}^{m \times n}$ is a vectors of feature-sets for each of the $m$ training samples and $\Y \in \mathbb{R}^m$ is a vector of corresponding labels (maximum SU allocation power). Here, $m$ is the number of training samples and $n$ is the number of \textit{features} in each sample.
\eat{
\begin{equation}\label{eq:XY}
    \X = \begin{bmatrix}
    \smallCap{X}_{\scriptsize{1}}^T\\
    \smallCap{X}_{\scriptsize{2}}^T\\
    \vdots\\
    \smallCap{X}_{\scriptsize{m}}^T
    \end{bmatrix}
    ,\quad
    \Y = \begin{bmatrix}
    y_1, y_2, ..., y_m
    \end{bmatrix}
\end{equation}}
The training process can be looked upon as an (typically convex) optimization in which the  \textit{training loss} objective is defined as:
\begin{equation}
\label{eq:SymLoss}
    \textbf{J}(\boldsymbol{\theta}) = \frac{1}{m} \sum_{i=1}^{m}{\textit{l}(\hat{y_i}, y_i, \boldsymbol{\theta})}
\end{equation}
where $y_i$ is the "ground truth", $\hat{y_i}=\A(\smallCap{X}_i)$ is the predicted value, and $\boldsymbol{\theta}$ is the internal set of the ML's parameters (coefficients and functions) to be learnt. 
Loss function, \textit{l}(.), defines the error for a single sample, and typically, 
the Mean Squared Error (MSE) $\textit{l}(\hat{y_i}, y_i) = \left\Vert  \hat{y_i} - y_i \right\Vert^2$ function is used. MSE is a good choice especially in our context because it is a convex function
 and has a positive second derivative; in particular, it penalizes samples with higher errors more than those with less errors. The training process provides us a $\boldsymbol{\theta}$ that minimizes the training loss $\textbf{J}(\boldsymbol{\theta})$.
 \eat{i.e., 
\begin{equation}
\label{eq:argminLoss}
    \operatorname*{argmin}_{\boldsymbol{\theta}}\quad \textbf{J}(\boldsymbol{\theta})
\end{equation}}
%We can later use $\boldsymbol{\theta}$ to predict new samples.

%\input{sections/learning/standard_techniques}

 
 \eat{
 
The reason behind the boost in performance from a deeper network, is that a more complex, non-linear function can be learned. Given sufficient training data, this enables the networks to more easily discriminate between different classes.
As numerAs Vision studies have shown over years[ref??], the deeper the model is the better, the performance you will usually achieve for a complex problem.
There are, though, two major challenges with very deep models. First, as the number of convolution layers increases, the number of trainable parameters increases drastically(??what order). Consequently, the computation cost of such models will also increase
. More importantly, the model is more likely prone to overfits. Much bigger dataset is a solution to address this problem but this sounds impossible for cases, including ours, where labeling cost is too high.}

\bluee{One way to avoid having a huge dataset and taking advantage of deep models is using other models where they have been well-trained for other problems like image classification, image localization, or etc.
As these model have been trained to classify images with multiple objects (~1000), there is a good chance that their feature maps (convolution filters) can be used for detecting vital information in other different purposes. We only have to fine-tune the model over our limited dataset with a much smaller learning rate.}

\bluee{Now, we can introduce our deep model idea. Despite the fact that some models like VGG[], ResNet[], Xception are trained over 1 million different images, they may not be optimized for our case as our image-like inputs include only preliminary objects like circles while they have been trained for more complicated objects like cats, cars, human, and etc. This does not mean our inputs are easier to process specially when the number of objects increases and they start to intersect into each other. Moreover, we are also interested about inter-object information like relative distance between each pair of objects. The idea is assuming a theoretical propagation model that fits the reality the most and create as many possible samples (images) as we want and train our deep model. Then we can use this trained model as a pre-trained model to fine tune it over our limited dataset. This way, we hope to improve our final model drastically.}
 
 
 
 
 
 Minimizing overall training cost is of paramount importance in our context,
as labeling a training sample can be expensive. 
In general, the training cost is expected to be largely proportional to the number of combinations of entity {\em locations} used, as varying entity powers should
incur negligible cost relatively.
%%%%
Minimizing training cost can also be interpreted as maximizing performance; given a set of training samples, the goal is to train the best possible model.



\para{Log-Distance Propagation Model.} 
We start with comparing the performance (in terms of \perr metric) of the algorithms for the case of Log-Distance propagation
model. See Fig.~\ref{fig:log}. We observe that \blue{\name} outperforms \svr and \nn approaches after a minimal number of training examples, for both the \pset and \sset cases, with the algorithms generally performing better with an increase in the number of samples. The performance of the algorithms also
improves with an increase in the number of SSs or PUs, as more PUs or SSs encode more information about
the environment (or path loss). Across the two settings \pset and \sset,
the performance of algorithms in \pset is better than that in \sset, since fundamentally the \pset has more direct information relevant to the spectrum allocation function.
%%%%%%%
Also, we note that, in the Log-Distance model, 
\ip performs very well--- which is not surprising as it has 
perfect/full knowledge of the underlying propagation model, and it has available 
{\em both} PUs parameter values as well as
the SS readings (and thus, is same in \pset and \sset)--while the 
ML techniques use only one of them 
depending on the setting. Note that \ip doesn't use any training, and hence, is shown to be
constant for a varying number of training samples. 
It is important to note that \blue{\name} is able to perform reasonably
close to \ip after 8k training samples--which suggests that \blue{\name}
 is able to 
learn the spectrum allocation function effectively. 

\para{Longley-Rice Propagation Model.}







\para{\blue{CNNs.}}
\blue{CNNs}, first introduced in \cite{fukushima1980neocognitron}, is a deep learning algorithm that has proved its ability to successfully capture the spatial and temporal dependencies among objects~\cite{cnnObjectDetecting} in an image via trainable filters. It performs the learning via non-linear transformations implemented as a series of 
nested layers.
The input data needs to be represented as a multidimensional data array; e.g. time-series signal strength can be seen as a 1D array with samples taken at regular time intervals, images can be represented as a 2D array of pixel values, videos can be represented in a 3D structure, etc. 
Then, a series of \textit{hidden layers} extract several abstract features, as an input to the next layer.
Each layer consists of several \textit{filters} that perform a convolution over the layer input; these layers  are  referred to as \textit{convolution layers}.
%%%%%%%%%%%%%%%%%%%%
Filters are feature detectors that convolve over the input and produce a transformed version of the data at the output. The filters are of the same dimensions as that of the input data, with their sizes varied based on the application; the filters
are learned through a training process called \textit{back-propagation}.
%%%%%
Normally, a non-linear \textit{activation function} is applied to layer's output just before feeding to the next layer, to handle the non-linearity of the input data. 
The output of the last convolution layer is "flattened" to feed into another set of layers called \textit{fully-connected layers}. See Fig.~\ref{fig:cnn_model} for an example.
Unlike the convolution layers which are responsible for extracting features and other important aspects of the image, fully-connected layers aim to predict the desired label, i.e., SU's allocated power in our case, based on the features detected by
the convolution layers.

%%%%%%%%%%%%%%%%%%%%%
\blue{CNN} has  been largely used to classify images or to analyze visual imagery existing in images.
\blue{CNN} can be efficient in detecting shapes and objects in images by first detecting smaller parts and then
spatially correlating them to classify bigger objects.
Essentially, the initial layers identify smaller features and 
feed a reduced input size (using maximum/average poll) to the next layer and so on.
Thus, the higher layers work with inputs with less lower-level details but with
more high-level information (detected features).















begin{comment}
\begin{wrapfigure}{r}{2in}
  \vspace{-0.5in}
  \hspace{-1.3in}
\includegraphics[width=5in]{figures/DesiredGain.pdf}
\vspace{-1.2in}
\caption{Observed vs.\ Desired Path Loss.}
\vspace{-0.2in}
\label{fig:desired}
\end{wrapfigure}
\end{comment}




\begin{comment}
\para{Why a learning-based approach?}
Most approaches, as mentioned in \ref{sub:related}, either assumes or estimates a propagation model/function to accomplish the spectrum allocation job successfully.
As even the well known propagation models suffer from accuracy, estimating it also entails a huge and probable unnecessary cost (either done by a thorough survey or through a fine grained spectrum sensors). 
An alternative way, then, is to learn SA function directly when there is no information about path-loss.



\para{Why not unsupervised?}
The learning should be a supervised model since our problem is defined as a regression problem.
More importantly, even if we convert the spectrum allocation to a classification problem (i.e. approving an SU request at a location with a demanding power), a sample without its label has no information regarding the SA function. 
% we still need to label the training samples.
Imagine PUs information is static, then, the only informative features are SU parameters.
As you can see, a specific SU request leads to a different cluster (class) in two different PUs settings (when PURs' thresholds are different).
Thus, we cannot apply unsupervised model to accurately separate SU requests.
We apply standard machine as well as deep (CNN) learning to achieve the goal.




\para{Why not RL?}
RL, in one hand, is not a suitable option since it is used to maximize long-term, {\em cumulative} spectrum allocation efficiency over time by exploiting the behaviour of SUs and/or PUs. 
The way we defined the spectrum allocation problem, on the other hand, is to maximize the short-term (instant) spectrum utilization in a greedy fashion.
% works as a spectrum overlay where inactivity of PUs is caught in a opportunistic manner.
%  Although RL approach is maximizing {\em cumulative} spectrum utilization over time by exploiting arrival patterns of the SUs,
% it may be useful to handle {\em simultaneous} SU requests.
% — we discuss this towards the section’s end.

Thus, learning the SA function skips the propagation model completely and lead us directly to our goal, the maximum power value being allocated to SU.

More detailed, upon requesting an SU at a location, we wish to use current system state (PUs and/or SSs information) to train a machine/deep learning model which performs the SA function.
The trained model can be later used to predict the upcoming requests.
We first design the model for a single SU and then extend it to multiple SUs.
Generally and for multiple SUs, we can store previous SUs and treat them as PUs (not exactly because they may get lower priority). 
Refer to \S\ref{sec:learning} for more details.
 \end{comment}

==> sections/learning/discussion.tex <==
\blue{\subsection{Discussion}
\label{sec:discussion}
practical implications:
\begin{itemize}
    \item PUs' Interference Evaluation: To collect samples and in cases where we do not have access to PUs and their receivers, we need to evaluate a system to measure interference to PUs' receivers (SM intends to allocate maximum possible power to SUs without causing any interference). To do so, we need to simulate PUs and PURs by creating artificial ones and place them in desired places. We, then, have PUs to send a signal (a known message) to their own PURs. Now, we start sending a signal from an SU (in a specific location). We change (increase) the power level till the point one of the artificial PUR is unable to retrieve its PU's message. 

    \item High training cost: Training, due to collecting and labeling the data samples, may be substantial but it is done just one time (survey duration defines the accuracy of collected data). Also, we can automate the process by using drones (or robots) to displace the elements.
\end{itemize}
}

==> sections/learning/eaten.tex <==


across the SUs.
See Fig.~\ref{fig:fairness}(b)-(c).
We observe that as desired the fair approach \namef has the best fairness metric, while 
having only a small disadvantage in the total power allocated. The greedy approach \nameg
yields the highest total power allocated.

\softpara{Spectrum Utilization (Data Rate).}
Finally, we compare the performance of our approaches in terms of the overall spectrum
utilization which we model using achievable data rate as follows. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
For each SU, we assign a receiver in a random location around the SU, and 
estimate the data rate that can be achieved between the SU and the receiver in presence of
the interference from PUs and other SUs. To compute achievable data rate, we calculate the 
SINR (signal-to-interference-plus-noise) ratio at the receiver, and use Shannon's capacity 
law to estimate the achievable data rate as $B\log_{2}(1 + \frac{S}{N + I})$ where 
$B$ is the channel bandwidth (1MHz here), $S$ is the average signal strength (received power), 
$N$ is the average noise, and $I$ is the interference.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
See Fig.~\ref{fig:fairness}(c), which plots the average data rate achieved by the SUs. 
As expected, we observe that the \nameg approach performs the best, 
which validates our weighted-subarea based greedy approach.
In this experiment, we moved the receiver to various locations around the SU 
within a distance of 100m.






\para{Handling SUs One at a Time.}
To handle subsequent SUs, we can augment the list of features to include the active SUs' parameters, and train the model accordingly. 
%%%%%%
This approach is viable, especially in the context of our \name model,
since active SUs with their parameters (location and allocated power) can 
easily be represented in the single input sheet dedicated to SUs. The only
change we need to make is that we must now represent SU's allocated power
too; we can represent them with a disk similar to PUs, i.e., with the
center's brightness and radius proportional to the allocated power. 
%%%%%%%%%%%%%%%%
%The other ML techniques can also be similarly extended to handle 
%subsequent  SUs one at a time.
%%%%%%%%%%%
\bluee{If multiple SU requests arrive \textit{together}, then to use the above
approach, we need to decide on an order in which to handle the requests.
One simple way is to handle them in a 
random order; we refer to this as \namer. We discuss two more ordering
approaches below.}

\softpara{{\tt \nameg} and {\tt -Fair} Ordering of SUs.}
In \nameg, we divide the whole area into non-overlapping subarea, and assign each subarea $X$ a weighted score equal to the total aggregated power transmitting from all the PUs and 
active SUs in $X$ or its adjoining cells.
%%%%%%
Then, we pick the SU requests in the ascending order of the weight of the subarea 
they belong to.
%%%%
%In our evaluations (\S\ref{sec:evals-multi}), \nameg outperforms \namer.
In the above \nameg approach, some SUs 
may not be allocated any power (e.g., if they are located near an SU already allocated optimal
power). To address this unfairness issue for simultaneous multiple SUs, 
we modify the \nameg approach as follows to design a fair scheme
\namef. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
If the allocated power to the requesting SU $x$ is less than a certain threshold, 
then we ``backtrack'' and reduce the allocated power of some of the 
previously-allocated SUs. In particular, we reduce the power of the SUs
"near" $x$ in proportion to their individual impact in improving the power allocation 
to $x$; we skip tedious details.
%%%%%%%
This results in ``freeing'' up some spectrum for allocation to $x$. 
%%%%%%%%%%%%%%%%%
Note that, the low power allocation to $x$ could also be due to it being very 
close to some PUs, in which case nothing can be done.

\input{sections/rnn_system} %Figure.


\para{Handling SUs One at a Time.}
To handle subsequent SUs, we can augment the list of features to include the active SUs' parameters, and train the model accordingly. 
%%%%%%
This approach is viable, especially in the context of our \name model,
since active SUs with their parameters (location and allocated power) can 
easily be represented in the single input sheet dedicated to SUs. The only
change we need to make is that we must now represent SU's allocated power
too; we can represent them with a disk similar to PUs, i.e., with the
center's brightness and radius proportional to the allocated power. 
%%%%%%%%%%%%%%%%
%The other ML techniques can also be similarly extended to handle 
%subsequent  SUs one at a time.
%%%%%%%%%%%
\bluee{If multiple SU requests arrive \textit{concurrently}, then to use the above
approach, we need to decide on an order in which to handle the requests.
One simple way is to handle them in a 
random order; we refer to this as \namer. We discuss two more ordering
approaches below.}

\softpara{{\tt \nameg} and {\tt -Fair} Ordering of Concurrent SUs.}
In \\ \nameg, we divide the whole area into non-overlapping subarea, and assign each subarea $X$ a weighted score equal to the total aggregated power transmitting from all the PUs and 
active SUs in $X$ or its adjoining cells.
%%%%%%
Then, we pick the SU requests in the ascending order of the weight of the subarea 
they belong to.
%%%%
%In our evaluations (\S\ref{sec:evals-multi}), \nameg outperforms \namer.
In the above \nameg approach, some SUs 
may not be allocated any power (e.g., if they are located near an SU already allocated optimal
power). To address this unfairness issue for simultaneous multiple SUs, 
we modify the \nameg approach as follows to design a fair scheme
\namef. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
If the allocated power to the requesting SU $x$ is less than a certain threshold, 
then we ``backtrack'' and reduce the allocated power of some of the 
previously-allocated SUs. In particular, we reduce the power of the SUs
"near" $x$ in proportion to their individual impact in improving the power allocation 
to $x$; we skip tedious details.
%%%%%%%
This results in ``freeing'' up some spectrum for allocation to $x$. 
%%%%%%%%%%%%%%%%%
Note that, the low power allocation to $x$ could also be due to it being very 
close to some PUs, in which case nothing can be done.

\input{sections/rnn_system} %Figure.

\para{Handling Multiple SUs Concurrently.}
\bluee{So far, we have allocated power in a greedy way; one SU at a time even if all the requests come at the same time. For obvious reasons, this approach may be neither fair nor optimal in terms of total allocated power to SUs. In this section, we consider allocating power to a set of demanding SUs concurrently without any ordering among them. We first propose an algorithm how to efficiently find the near-optimal total power allocated to SUs and then discuss ways of incorporating new machine learning models to generate the power values for each SU.}

\bluee{To create the ground truth that can be later used for training, we develop a binary-search-like algorithm where a set of SUs are allocated a power such that it is fair and total power is maximized. See Algorithm~\ref{alg:multi_sus_conc}.
In this algorithm, it is always assumed that the set of $Low$ power levels is interference-free to PUs. 
Initially, $Low$ is filled with noise floor which obviously cannot cause any interference.
$High$ array is also initialized with a very high value that even a single SU can cause interference. At each step, we take the SU whose remaining range ($high - low$) is the maximum and tries to shrink it.
We take the average of the high and low values and along with other $Low$ values we test if the new value causes interference.
The algorithm stops when the difference between lower and higher bound of all SUs is less than $\epsilon$.
The time complexity of the algorithm is $O\big((MaxPower - NoiseFloor) * \epsilon\big)$. }

\bluee{As stated earlier, the CNN models were trained to predict the maximum power available for the requesting SU, given all PUs and other active SUs. This power values can be totally different and undervalued than those returned by Algorithm~\ref{alg:multi_sus_conc}. To reach to the new power levels, we propose to, first, predict the maximum power level for each SU separately (i.e. single SU) and then re-adjust the maximum power values altogether.
We propose two solutions to make this transition.}
\bluee{
\begin{enumerate}
    \item \textbf{Simple NN.} The simplest model that can accomplish the transition is a multi-outputs neural network model with a small number of layers and neurons. 
    The input, to this model, is the set of SUs including their location and the predicted power (the output of the CNN model for single SU) and the output is the set of adjusted power values. 
    The NN output is feed with the output of Algorithm~\ref{alg:multi_sus_conc} in training phase.
    A benefit of using NN is it does not pick any ordering (biases) among SUs. We train the model with a maximum allowed number of SUs and the last places with dummy values if the real number of SUs is smaller.
    In our simulations, we used 4 layers with each has 128 neurons and a dropout of 80\% before the last layer.
    \item \textbf{RNN.} The goal is to adjust the power level of a set of SUs which can be interpreted as changing a sequence of SUs to a new sequence. In NLP world and to translate a text from a language to another, special Recurrent Neural Networks (RNN) models are used called \textit{Seq2Seq}. Recurrent Neural Networks is a class of neural networks that is suited for handling sequential data where the current prediction (an SU request here) depends on previous (and possible next) inputs.
    The way it works is it memorizes the previous (next) inputs via some internal mechanisms. \textit{Seq2seq} models comprises an encoder, to encode the input sequence, and a decoder where the encoded input is changed to the target sequence.
    More specifically, we propose to use a bi-directional long short-term memory (LSTM) model, in the encoder side, and another LSTM in the decoder side. See Fig.~\ref{fig:rnn_system}. 
    LSTM model with the help of some internal gates (\textit{forget}, \textit{input} and \textit{output}) and a \textit{cell} state can remember how many SUs (with what allocated power level) has been processed. 
    The reason we use bi-directional LSTM is we do not want any ordering being imposed among SUs. 
    So, at any step and with the help of forward and backward LSTM, the model is aware of both previous and next SU requests. 
    Just like NLP models where words (or characters) are transformed into vectors of numbers, we can feed our \textit{seq2seq} model a vector. 
    More specifically, we take the predicted power value, by the \textit{DeepAlloc} model, and create another image for each SU separately.
    We then use the \textit{DeepAlloc} model to create our \textit{seq2seq} input with the difference that we drop the fully connected part and take the feature map of the last convolution layer of the model.
    The output is in the form of a vector. 
    We repeat this for each SU to construct the input SUs sequence and pass it through the encoder part.
    We can also provide PUs information by this way.
    The decoder, on the other hand, will generate the adjusted power level for all the SUs as the output sequence.
\end{enumerate}}


\begin{algorithm}
	\caption{Allocating power concurrently to SUs} 
	\label{alg:multi_sus_conc}
	\begin{algorithmic}[1]
	\State \textbf{Input:} $PUs$, $SUs$, $\epsilon$, Propagation Model.
	\State\textbf{Output:} Set $P$ of allocated powers to each SU s.t. the total is maximized.
	\State $Low \gets [NoiseFloor] * |SUs|$
	\State $High \gets [MaxPower] * |SUs|$
	\While{($any\big[High_i - Low_i > \epsilon$ for $0 \leq i < |SUs|\big]$)}
	    \State $Mid \gets Low$
	    \State $idx \gets \argmax_{i} High_{i} - Low_{i}$
	    \State $Mid_{idx} \gets \frac{High_{idx} - Low_{idx}}{2}$
	    \If{SUs with Mid causes interference}
	        \State $High_{idx} \gets Mid_{idx}$
	   \Else
	        \State $Low_{idx} \gets Mid_{idx}$
	   \EndIf
	\EndWhile
	\State \textbf{Return} $Low$
	\end{algorithmic} 
\end{algorithm}

\para{Multiple Channels; Request Durations.} 
Till now, we have implicitly assumed a single channel. 
To handle multiple channels, we can extend our schemes easily.
If the signal propagation characteristics are different for different channels,
then we can create a separate model for each channel.
Then, for a single-SU request, we can pick the channel that allows for maximum power allocation,
while for multiple SUs, we can modify the above approaches \nameg and \namef easily for the
multiple channels setting. The \nameg approach extends naturally. For the \namef approach, 
instead of just reducing powers
of previously-allocated SUs, we can also consider the option of channel-reassignment, but
for simplicity, we do not change assigned channels. \bluee{For \namenn and \namernn, we use a simple scheme of uniformly (and randomly) partitioning the given set of SUs into multiple sets and assign a channel to each set; incorporating channel assignment in the model would require much more training, and thus not considered for simplicity.}
%%%%%
Finally, to handle requests for a specified duration, 
we reallocate active requests whenever
an SU becomes inactive (i.e., at the end of its request duration).

==> sections/learning/other_challenges.tex <==
\subsection{Challenges}
\label{sub:challenges}

As for all machine learning applications, the first challenge is how to avoid overfitting/underfitting.
In static PUs configuration, for example, the only informative parameters are SU location and power. There is a high chance that any ML algorithm tends to underfitt in this setting.
As mentioned before, we can circumvent this issue by introducing more non-linear combination of features.
For instance and because distance play a vital role predicting the maximum allocated power, we can create features like $x^2$, $y^2$, or $x^2+y^2$ where $x$ and $y$ are the values for SU location in different axes.
We, however, should be careful adding more complexity to our problem since the learning can suffers from overfitting.
This is more important when collecting and labeling more samples has a huge cost just like in our case.
Designing the ML and CNN architectures plays an important role as high number of layers in NN, high number of filters and parameters in the last layer in CNN, high amount of newly introduced features in LR, and high amount of support vectors in SVR cause overfitting.

Talk about hyper-parameters. The second challenge is choosing proper kernels(activation functions) in our purpose. 
As discussed before, some non-linear activation function like ReLU fits better in the initial layers while linear functions seems the best possible candidate for the last layer.

==> sections/learning/standard_techniques.tex <==
\subsection{Standard Regression Techniques} 
\label{sub:standard}

Learning the SA function as described above is essentially a supervised regression learning process, and there are
various standard algorithms such as Linear Regression (LR), Neural Networks (NN), and Support Vector Regression (SVR). We briefly discuss how these techniques can be applied to our context. We implement and evaluate these techniques in \S~\ref{sec:simulations} and~\ref{sec:testbed}.
%, we implement and evaluate the above techniques for learning the spectrum allocation function.

\softpara{Linear Regression (LR).}
LR \iab{is} one of the simplest techniques to solve regression problems, wherein the label is expressed as a linear combination of features; the \iab{learned} linear coefficient represents the different weights \iab{of} the features. More generally and to achieve non-linearity, the label may be represented as a linear combination of higher (or lower) order polynomial terms.

\softpara{Neural Networks (NNs).}
NNs are composed of layers of neurons each of which is computed as some non-linear function of the sum of its inputs; the non-linear activation functions facilitate learning the non-linearity of our SA function \A effectively.
%%Different layers with sufficient number of neurons along with a kernel combined together receive PUs (or SSs) information and predict maximum power a requesting SU can have.
%%%Note that the last layer will have only one neuron and its kernel should be linear since the output is a real number that can be both negative and positive (power is represented in dB).

\softpara{Support Vector Regression (SVR).}
Support Vector Machine (SVM) are supervised learning models that analyze data used for classification and regression analysis. SVMs can efficiently perform a non-linear classification using what is called the kernel trick, implicitly mapping their inputs into high-dimensional feature spaces. Support Vector Regression (SVR)  is a regression counterpart of SVMs. SVRs use essentially the same technique as SVMs except that the hyperplane used to separate the classes in SVM is now used as a regression function in the SVRs~\cite{drucker1997support, smola2004tutorial}; for the technique to 
be effective, additional constraints are added so that the given training data points are close enough to the hyperplane.



\begin{comment}
In SVR, almost the same algorithm applies with a slight difference that the curve is used to predict the real output with aid of support vectors 
In another words, one or more than one support vectors will be used to map the input to a position on the curve which is not further than a $\epsilon$ from the real output.
That means, we get the closest value to the actual curve when the distance between the support vectors and the regressed curve is maximized.
The way SVR works seems be one of the ML technique for our problem.


takes the inputs to a higher hyper-plane ($> N$) where $N$ is the dimension of the inputs. As we know, SVM minimizes the error by finding a curve, which is achieved from a (non) linear kernel like RBF \cite{han12}, that splits samples belonged to different classes with maximum margin between the curve and classes in classification problems.
\end{comment}

==> sections/results/conservative.tex <==
\begin{figure}%
    \vspace{-0.2cm}
    \centering
    \subfloat{{\includegraphics[width=.98\linewidth]{figures/conserve_legend.png} }}%
    % \qquad\hspace{-0.2in}
    \vspace{-0.6cm}
    \setcounter{subfigure}{0}
    \subfloat[\pset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_splat_100grid_10cell_conserve.png} }}%
    \qquad\hspace{-0.2in}
    \subfloat[\sset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_splat_100grid_10cell_conserve_ss.png} }}%
    \vspace{-0.1in}
    \caption{Handling multi-path effect by considering a more conservative allocation function. The plot shows \perr and \pfp metrics for the learnt basic and conservative functions.}%
    \label{fig:conservative}%
    \vspace{-0.1in}
\end{figure}

==> sections/results/false_positive.tex <==
\begin{figure}%
    \vspace{-0.4cm}
    \centering
    \subfloat[\pset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_splat_100grid_10cell_assymetric.png} }}%
    \qquad\hspace{-0.2in}
    \subfloat[\sset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_splat_100grid_10cell_assymetric_ss.png} }}%
    \vspace{-0.2cm}
    \caption{Minimizing false positive error (\pfp).}
    \label{fig:false_positive}%
    \vspace{-0.5cm}
\end{figure}

==> sections/results/log.tex <==
\begin{figure*}[t]%
    \vspace{-0.2in}
    \centering
    \begin{minipage}[t]{1\textwidth}
    \hspace{-0.1cm}
    \subfloat{{\includegraphics[width=.46\textwidth]{figures/legends.png} }}
    \hspace{0.2cm}
    \subfloat{{\includegraphics[width=.46\textwidth]{figures/legends.png} }}
    \vspace{-0.45cm}
    \setcounter{subfigure}{0}
    \subfloat[\pset with increasing number of training samples and 10-20 PUs.]{{\includegraphics[width=.23\textwidth]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell.png} }}%
    \qquad\hspace{-0.16in}
    \subfloat[\pset with increasing number of PUs and \bluee{2k} training samples.]{{\includegraphics[width=.23\textwidth]{figures/Changing_PUs_number_log_alpha3_1000grid_1cell.png} }}%
    % \vspace{-0.2cm}
    % \caption{Log-Distance Propagation model using PUs' information.}%
    % \label{fig:log_pus}%
% \end{figure}
% \begin{figure}
    % \newline
    % \vspace{-0.2cm}
    % \centering
    \qquad\hspace{-0.16in}
    \subfloat[\sset with increasing number of training samples and 10-20 PUs.]{{\includegraphics[width=.23\textwidth]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell_using_sensors.png} }}%
    \qquad\hspace{-0.16in}
    \subfloat[\sset with increasing number of SSs and \bluee{2k} training samples.]{{\includegraphics[width=.23\textwidth]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell_changing_number_sensors.png} }}%
    \vspace{-0.1in}
    \caption{Performance comparison of various techniques with Log-Distance as the underlying signal propagation model.}
    \label{fig:log}
    \end{minipage}
    \vspace{-0.3cm}
\end{figure*}

==> sections/results/log10_20pus_1_4sus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_1_4SUs_1000m_alpha3_noise1_1000grid_1cell.png}
    \vspace*{-0.2in}
    \caption{Log-distance propagation 10-20PUs, 1-4SUs} 
    \label{fig:log_4sus}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/log_10_20pus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell.png}
    \vspace*{-0.2in}
    \caption{Log-distance propagation 10-20PUs} 
    \label{fig:log_10_20pus}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/log_changing_sensors.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell_changing_number_sensors.png}
    \vspace*{-0.2in}
    \caption{Log-distance propagation 10-20PUs, changing number of sensors} 
    \label{fig:log_10_20pus_sensors}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/log_pus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    {
        \includegraphics[width=0.5\textwidth, center]{figures/Changing_15PUs_1000m_alpha3_noise1_1000grid_1cell.png}
    }
    {
        \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_1000m_alpha3_noise1_1000grid_1cell.png}
    }
    
    \vspace*{-0.2in}
    \caption{Log-distance propagation using PUs, (top) 15 PUs, (bottom) 10-20PUs} 
    \label{fig:log_pus_old}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/multi_sus_multi_chan.tex <==
\begin{figure*}[t]%
    \vspace{-0.4cm}
    \begin{minipage}[t]{1\textwidth}
    \centering
    \hspace{0.5cm}
    \subfloat{{\includegraphics[width=1\textwidth]{figures/channels_legend.png} }}
    % \hspace{0.5cm}
    % \subfloat{{\includegraphics[width=.46\textwidth]{figures/legends.png} }}
    \vspace{-0.45cm}
    \setcounter{subfigure}{0}
    \subfloat[Single Channel. Total allocated power to multiple (5) SUs.]{{\includegraphics[width=.23\textwidth]{figures/Changing_PUs_number_splat_100grid_10cell_single_chan_multi_sus_tot.png} }}%
    \qquad\hspace{-0.16in}
    \subfloat[Single Channel. Max/min allocated power to SUs.]{{\includegraphics[width=.23\textwidth]{figures/Changing_PUs_number_splat_100grid_10cell_single_chan_multi_sus_max_min.png} }}%
%     \vspace{-0.2cm}
%     \caption{Log-Distance Propagation model using SSs' information.}%
%     \label{fig:log_sss}%
% \end{figure}
% \begin{figure}
    % \vspace{-0.2cm}
    % \centering
    \qquad\hspace{-0.16in}
    \subfloat[4 Channels. Total allocated power to multiple (20) SUs.]{{\includegraphics[width=.23\textwidth]{figures/Changing_PUs_number_splat_100grid_10cell_multi_chan_multi_sus_tot.png} }}%
    \qquad\hspace{-0.16in}
    \subfloat[4 Channels. Maximum/minimum allocated power to SUs (20).]{{\includegraphics[width=.23\textwidth]{figures/Changing_PUs_number_splat_100grid_10cell_multi_chan_multi_sus_max_min.png} }}%
    \vspace{-0.2cm}
    %\caption{Performance comparison of various techniques in terms of \perr (dB) metric in an area with Longley-Rice as the underlying signal propagation model.}
     \vspace{-0.05in}
    \caption{Fairness and Multiple Channels.}
    \label{fig:multi_sus_chann}
    \end{minipage}
    \vspace{-0.2in}
\end{figure*}

==> sections/results/splat_10_20pus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_splat_100grid_10cell.png}
    \vspace*{-0.2in}
    \caption{splat propagation 10-20pus} 
    \label{fig:splat_10_20pus}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/splat_changing_sensors.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_splat_100grid_1cell_changing_number_sensors.png}
    \vspace*{-0.2in}
    \caption{splat propagation 10-20pus, changing number of sensors} 
    \label{fig:splat_changing_sensors}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/splat_pus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    {
        \includegraphics[width=0.5\textwidth, center]{figures/Changing_15PUs_splat_100grid_10cell.png}
    }
    {
        \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_splat_100grid_10cell.png}
    }
    
    \vspace*{-0.2in}
    \caption{splat propagation 15pus} 
    \label{fig:splat_pus_old}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/splat_sus.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_1_4SUs_1splat_1000grid_1cell.png}
    \vspace*{-0.2in}
    \caption{splat propagation 10-20pus, 1-4sus} 
    \label{fig:splat_sus}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/splat_using_sensors.tex <==
% * how it works
\begin{figure}[h]
    %\centering
    %\vspace*{-1.1in}
    %\includegraphics[width=0.4\textwidth, center]{figures/cnn-raj.pdf}
    \includegraphics[width=0.5\textwidth, center]{figures/Changing_10_20PUs_splat_1000grid_1cell_400sensors.png}
    \vspace*{-0.2in}
    \caption{splat propagation 10-20pus, 1su, using 400 sensors} 
    \label{fig:splat_using_sensors}
    \vspace*{-0.2in}
\end{figure}

==> sections/results/su_power_adjustment.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[t]{1\linewidth}
    \includegraphics[width=0.9\textwidth, center]{figures/su_power_adjustment.png}
    \vspace{-0.2in}
      \caption{SUs before (left) and after (right) power re-adjustment. PUs are not included for the sake of simplicity.}
   \label{fig:su_readjust}
   \vspace*{-0.1cm}
\end{minipage}
\hspace{0.1in}
   \vspace{-0.1in}
\end{figure}

==> sections/results/sus.tex <==
\begin{figure}%
    \centering
    \vspace{-0.4cm}
    % \subfloat{{\includegraphics[width=.6\linewidth]{figures/sus_legend.png} }}%
    % \qquad\hspace{-0.2in}
    % \vspace{-0.55cm}
    \setcounter{subfigure}{0}
    \subfloat[\pset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_1_10SUs_1splat_1000grid_1cell.png} }}%
    \qquad\hspace{-0.2in}
    %  figures/Changing_10_20PUs_1_10SUs_1splat_1000grid_1cell_ss.png
    \subfloat[\sset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_1_10SUs_1splat_1000grid_1cell.png} }}%
    \vspace{-0.2cm}
    \caption{Evaluating techniques for allocating power to {\em subsequent} SUs, when other SUs may be active.}
    %The \perr for \ip in Longley-Rice model is 21.38 dB (not shown for clarity) \blue{should we remove the last sentence? we already have it in the text}.}
    \label{fig:sus}%
    \vspace{-0.3cm}
\end{figure}

==> sections/results/sus_datarate.tex <==
\begin{figure}%
    \centering
    \vspace{-0.2in}
    \subfloat{{\includegraphics[width=.9\linewidth]{figures/sus_datarate_legend.png} }}%
    % \qquad\hspace{-0.2in}
    \vspace{-0.4cm}
    \setcounter{subfigure}{0}
    \subfloat[\pset.]{{\includegraphics[width=.47\linewidth]{figures/Changing_10_20PUs_1_10SUs_1splat_1000grid_1cell_data_rate.png} }}%
    \qquad\hspace{-0.2in}
    % figures/Changing_10_20PUs_1_10SUs_1splat_1000grid_1cell_data_rate_ss.png
    \subfloat[\sset.]{{\includegraphics[width=.47\linewidth]{} }}%
    \vspace{-0.2cm}
    \caption{Overall spectrum utilization for multiple SUs. \bluee{PU-ASAP; SU-12pm.}} %simultaneous SU requests.}
    %The \perr for \ip in Longley-Rice model is 21.38 dB (not shown for clarity) \blue{should we remove the last sentence? we already have it in the text}.}
    \label{fig:sus_datarate}%
    \vspace{-0.1in}
\end{figure}

==> sections/results/testbed_sensor_density.tex <==
% \begin{figure}%
%     \centering
%     \vspace{-0.4cm}
%     \subfloat[\sset with increasing number of SSs and 520 training samples]{{\includegraphics[width=.47\linewidth]{figures/testbed_using_sss_changing_sensor_density.png} }}%
%     \vspace{-0.2cm}
%     \caption{\blue{Testbed. Effect of number of SSs}.}%
%     \label{fig:testbed_ss_dense}%
%     \vspace{-0.3cm}
% \end{figure}

\begin{figure}[h]
    %\centering
    %\vspace*{-0.4in}
    %\includegraphics[width=0.65\textwidth, center]{figures/DesiredGain.pdf}
    \includegraphics[width=0.5\linewidth, center]{figures/testbed/testbed_using_sss_changing_sensor_density.png}
    \vspace*{-0.2in}
    \caption{\sset with increasing number of SSs and 520 training samples.} 
    \label{fig:testbed_ss_dense}
    \vspace*{-0.4cm}
\end{figure}
